Underwater Robot Manipulation: Advances, Challenges and Prospective Ventures

Underwater manipulation is one of the most remarkable ongoing research subjects in robotics. \acp{I-AUV} not only have to cope with the technical challenges associated with traditional manipulation tasks but do so while currents and waves perturb the stability of the vehicle, and low-light, turbid water conditions impede perceiving the surroundings. Certainly, the dynamic nature and our limited understanding of the marine environment hinder the autonomous performance of underwater robot manipulation. This manuscript provides a discussion on previous research and the limiting factors that impose on the long-envisioned prospects of autonomous underwater manipulation to finally highlight research directions that have the potential to improve the autonomy capabilities of I-AUV.

==> Sections/5_future_research.tex <==
\section{FUTURE RESEARCH AVENUES \label{sec:future_research}}

% \cite{ardon2021building}

% \textcolor{red}{
%     \begin{enumerate}
%         \item \textit{Datasets}
%         \item \textit{Mobile base manipulation}
%         \item \textit{sensor fusion and handling of different data structure}
%         \item \textit{Exploring other paradigms for improvements in manipulation like those based on “learning by demonstration”}
%         \item \textit{Visibility}\\
%         Low-visibility - The use of high intensity LEDs improve the detection of the markers using optical sensors like cameras, where visibility is not optimal, as in smoke-filled environments or underwater in conditions where the water is turbid. Slightly positive buoyancy requires continuously spun thrusters resulting in poor visibility.   
%         \item \textit{Grasper}
%         \item \textit{Manipulator Position}\\
%         The AUV elements should be out of the arm workspace to avoid damages on failure of its autonomous control. When not  operative,  the  arm  should  adopt  a  position  that  minimizes the water resistance while the vehicle moves through the water.  
%         \item \textit{Dynamic Coupling}\\
%         Often experiments are conducted in tanks to avoid disturbances like currents as well as vehicle-arm coupling. If the  arm  weight  is  a  high  percentage  of  the  vehicle  weight, considerable dynamic coupling between both subsystems  would  be  introduced.  
%         \item \textit{Time delay in Communication}\\
%         The principal obstacle in communicating with a generic AUV during a mission is the low bandwidth and a signiﬁcant time delay inherent in acoustic subsea communication.
%     \end{enumerate}
% }

% - A fruitful area of future work would be to implement a more physically based scattering model, such as the Kirchhoff approximation (Abawi, 2016).
% - resolve identified challenges, including computational complexity in our MPC implementation associated with CLRRT
% - Cooperation between multiple UVMS
% - increasing the autonomy levels of an underwater intervention system
% - explore other paradigms for improvements in manipulation like those based on “learning by demonstration”
% - Estimating distance from camera
% - Tasks with priori trajectory are easy, more work for those without unknown path
% - When visual feedback is required i.e. grasping, plugging a connector, current vision is limitted to quasi-planar objects for which an image before intervention is required
% - High arm velocities NOT considered
% - Vehicle-arm coordination NOT addressed
% - remote controllers  react to problems in a timely manner
% - Only a few practical setups have been reported to reproduce only in normal environment
% Robot-environment interaction is evidently very important in 
% order to obtain behaviour similar to the real situation; for 
% example, when the robot touches the seafloor, this event is not 
% a simple collision, but it triggers other events that influence 
% the state of the environment (losing of visibility caused by the 
% powder). The last example, suggests that the collision 
% detection and response are just a subset of information needed 
% in a realistic simulation that involves vision, for this reason an 
% accurate scene synthesis is not only an aesthetic feature, but 
% represents an important aspect. In the natural world there are a 
% large variety of environments and conditions that needs to be 
% simulated and that can provide a powerful tool to minimize 
% time and costs for the development of this kind of application. 
% Finally, it is noticeable that the work here presented shows 
% only the first step in the progress direction towards the long 
% term objective, described in the introduction section.        


==> Sections/accomplishedtasks.tex <==
\section{ACCOMPLISHED TASKS}
\begin{enumerate}
  \item Autonomous inspection of an underwater structure
  \item Autonomous location, cleaning, and inspection of an anchor chain
  \item Autonomous grasping and turning of a valve from swimming, undocked vehicle
\end{enumerate}

==> Sections/datacollection.tex <==
\section{DATA COLLECTION}

A new 3D underwater laser scanner has been presented to demonstrate advanced technique of data collection [cite: 3D Laser Scanner for Underwater Manipulation]. The  object  3D  structure  is  recovered  by  using  a laser stripe emitter combined with a camera. The laser emitter is  mounted  on  a  robot  arm  that  is  in  charge  of  performing the scanning motion and relating the laser plane with respect to  the  camera  pose.  A  3D  point  cloud  is  generated  after  the scanning process, and combined with a grasp region indicated by an operator on a 2D view of the target object. This allows to reduce the number of 3D points and to delimit the grasping area.  After  that,  a  grasp  planner  computes  a  suitable  grasp on  the  reduced  point  cloud,  and  an  inverse  kinematic  solver computes a suitable vehicle-arm pose for reaching the object at the desired grasp pose. All the previous methods have been validated both in simulated and real conditions in a water tank. The proposed approach could be applied for recovery missions in the sea with autonomous vehicles. 
In order to transform 3D coordinates of objects detected by the camera into the manipulator reference system, the camera must be externally calibrated with respect to the manipulator  base  link  (known  as  eye-hand  calibration).This is done by attaching a checker board pattern (whose model  is  known)  to  the  gripper  in  such  a  way  that  the pattern  origin  is  in  a  known  pose  with  respect  to  the arm end-effector. This allows the whole kinematic chain,from  the  arm  base  link  to  the  pattern  origin,  to  be computed. Then, the pattern is moved to different poses in the camera field of view, and an image is captured for each of them. Next, the intrinsic and extrinsic calibration parameters  are  computed  following  standard  calibration techniques (using the Matlab Calibration Toolbox in this case). This procedure has to be performed only once, and the  calibration  will  remain  valid  as  long  as  the  relative arm-camera position is not changed.
